Creativity in Robot Manipulation with Deep Reinforcement Learning

Deep Reinforcement Learning (DRL) has emerged as a powerful control technique in robotic science. In contrast to control theory, DRL is more robust in the thorough exploration of the environment. This capability of DRL generates more human-like behaviour and intelligence when applied to the robots. To explore this capability, we designed challenging manipulation tasks to observe robots strategy to handle complex scenarios. We observed that robots not only perform tasks successfully, but also transpire a creative and non intuitive solution. We also observed robot's persistence in tasks that are close to success and its striking ability in discerning to continue or give up.

==> OpenPoints.tex <==
1. Increase the vertical space between figures in the 'combined' plot. DONE
2. Re-plot the throw-grab plot-> change the condition for success to the new updated one, current one is wrong.
3. Add citations to the Introduction.
4. Check if citations are needed else-where.
5. Change all figure title/xlabel/ylabel, etc. to the same fontsize and fontface.
5. Set a uniform naming convention- grab/throw, punch/bounce, goal/target.
6. Write more about figure 3
